AURO: Reinforcement Learning for Adaptive User Retention Optimization in Recommender Systems

The field of Reinforcement Learning (RL) has garnered increasing attention for its ability of optimizing user retention in recommender systems. A primary obstacle in this optimization process is the environment non-stationarity stemming from the continual and complex evolution of user behavior patterns over time, such as variations in interaction rates and retention propensities. These changes pose significant challenges to existing RL algorithms for recommendations, leading to issues with dynamics and reward distribution shifts. This paper introduces a novel approach called \textbf{A}daptive \textbf{U}ser \textbf{R}etention \textbf{O}ptimization (AURO) to address this challenge. To navigate the recommendation policy in non-stationary environments, AURO introduces an state abstraction module in the policy network. The module is trained with a new value-based loss function, aligning its output with the estimated performance of the current policy. As the policy performance of RL is sensitive to environment drifts, the loss function enables the state abstraction to be reflective of environment changes and notify the recommendation policy to adapt accordingly. Additionally, the non-stationarity of the environment introduces the problem of implicit cold start, where the recommendation policy continuously interacts with users displaying novel behavior patterns. AURO encourages exploration guarded by performance-based rejection sampling to maintain a stable recommendation quality in the cost-sensitive online environment. Extensive empirical analysis are conducted in a user retention simulator, the MovieLens dataset, and a live short-video recommendation platform, demonstrating AURO's superior performance against all evaluated baseline algorithms.

==> offline_table.tex <==
\begin{table}[t]
    \caption{Results of offline experiments on MuJoCo tasks. Numbers are the normalized scores according to D4RL~\cite{fu2020d4rl}. ME, M, MR and R correspond to the medium-expert, expert, medium-replay and random dataset, respectively. Numbers after $\pm$ is the standard deviation across trials with four different seeds.}
    \label{tab:offline}
    \centering
    \scriptsize
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
~ & BCO & SOIL & CQL & MOPO & MAPLE & \makecell{MAPLE\\+DARA} & \makecell{MAPLE\\+SRPO} & \makecell{MAPLE\\+\algo} \\
\midrule
Walker2d-ME & 0.25±0.04 & 0.14±0.08 & \textbf{0.63}±0.13 & 0.06±0.05 & 0.14±0.08 & 0.31±0.02 & 0.22±0.07 & 0.29±0.12 \\
Walker2d-M & 0.17±0.07 & 0.16±0.01 & \textbf{0.75}±0.02 & 0.15±0.22 & 0.41±0.19 & 0.46±0.10 & 0.32±0.17 & 0.49±0.04 \\
Walker2d-MR & 0.01±0.00 & 0.04±0.01 & 0.06±0.00 & -0.00±0.00 & 0.13±0.01 & 0.12±0.00 & 0.13±0.01 & \textbf{0.14}±0.01 \\
Walker2d-R & 0.00±0.00 & 0.00±0.00 & 0.00±0.00 & -0.00±0.00 & \textbf{0.22}±0.00 & 0.16±0.01 & 0.22±0.00 & 0.22±0.00 \\
Hopper-ME & 0.08±0.02 & 0.01±0.00 & 0.20±0.07 & 0.01±0.00 & 0.45±0.07 & 0.49±0.01 & 0.43±0.06 & \textbf{0.51}±0.06 \\
Hopper-M & 0.00±0.00 & 0.08±0.00 & 0.29±0.06 & 0.01±0.00 & 0.38±0.09 & 0.26±0.02 & 0.48±0.04 & \textbf{0.71}±0.14 \\
Hopper-MR & 0.00±0.00 & 0.00±0.00 & 0.08±0.00 & 0.01±0.01 & 0.55±0.17 & 0.75±0.10 & 0.73±0.16 & \textbf{0.76}±0.08 \\
Hopper-R & 0.00±0.00 & 0.00±0.00 & 0.10±0.00 & 0.01±0.00 & 0.12±0.00 & 0.12±0.00 & 0.25±0.08 & \textbf{0.32}±0.00 \\
HalfCheetah-ME & 0.43±0.00 & 0.00±0.00 & 0.03±0.04 & -0.03±0.00 & 0.53±0.07 & 0.39±0.00 & 0.58±0.04 & \textbf{0.61}±0.02 \\
HalfCheetah-M & 0.14±0.02 & 0.39±0.00 & 0.42±0.01 & 0.36±0.27 & 0.61±0.01 & \textbf{0.66}±0.03 & 0.62±0.00 & 0.62±0.01 \\
HalfCheetah-MR & 0.16±0.01 & 0.25±0.00 & 0.46±0.00 & -0.03±0.00 & 0.52±0.01 & 0.53±0.02 & 0.54±0.00 & \textbf{0.56}±0.01 \\
HalfCheetah-R & 0.14±0.01 & 0.35±0.01 & -0.01±0.01 & -0.03±0.00 & 0.20±0.02 & 0.19±0.01 & \textbf{0.22}±0.00 & 0.21±0.00 \\
\midrule
Average & 0.11 & 0.11 & 0.25 & 0.04 & 0.36 & 0.37 & 0.40 & \textbf{0.45}\\
\bottomrule
    \end{tabular}
\end{table}

==> tex_includes/tab2.tex <==
% \begin{table*}[t]
%     \centering
%         \caption{Results of ablation studies in the modified KuaiSim simulator.}
%         \vspace{-0.2cm}
%     \label{fig:ablation}
% \scriptsize
% % \small
%     \begin{tabular}{l|c|c|c|}
%     \toprule
%         ~ & \rows{\makecell{Average Return\\ Days (↓)}}{\makecell{Return Probability at\\ Day 1 (↑)}}{\makecell{Retention\\Reward (↑)}}
%         % {\makecell{ Like Rate\\\textperthousand, ↑ }}{ \makecell{Comment Rate\\ \textperthousand, ↑ }}{\makecell{Unlike Rate\\ \%, ↓} }
%         \midrule
%         w/o exploration & \rows{1.868$\pm$0.061}{0.708$\pm$0.015}{-0.018$\pm$0.000}
%         w/o state abstraction & \rows{1.803$\pm$0.109}{0.732$\pm$0.034}{-0.018$\pm$0.001}
%         w/o value-based loss & \rows{1.672$\pm$0.208}{0.776$\pm$0.068}{-0.017$\pm$0.002}
%         \midrule
%         $n=3$ & \rows{}{}{}        
%         $n=5$ & \rows{}{}{}        
%         $n=6$ & \rows{}{}{}        
%         \midrule
%         AdaRec  & \rows{\textbf{1.541}$\pm$0.056}{\textbf{0.819}$\pm$0.017}{\textbf{-0.015}$\pm$0.001}
%         \bottomrule
%     \end{tabular}
% \end{table*}
